Interventional Probing in High Dimensions: An NLI Case Study

Probing strategies have been shown to detect the presence of various linguistic features in large language models; in particular, semantic features intermediate to the "natural logic" fragment of the Natural Language Inference task (NLI). In the case of natural logic, the relation between the intermediate features and the entailment label is explicitly known: as such, this provides a ripe setting for interventional studies on the NLI models' representations, allowing for stronger causal conjectures and a deeper critical analysis of interventional probing methods. In this work, we carry out new and existing representation-level interventions to investigate the effect of these semantic features on NLI classification: we perform amnesic probing (which removes features as directed by learned linear probes) and introduce the mnestic probing variation (which forgets all dimensions except the probe-selected ones). Furthermore, we delve into the limitations of these methods and outline some pitfalls have been obscuring the effectivity of interventional probing studies.

==> tables_figures/related_interventions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht!]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|llllll@{}}
\toprule
                                                                                                                    & Intervention                                                                                        & Tested Effect                                                                                            & Feature Characterisation                                       & \begin{tabular}[c]{@{}l@{}}Requires Intermediate \\ Labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}Intervention Linked to\\ Concept Interpretation\end{tabular} & Domain                \\ \midrule
Amnesic Probing / INLP                                                                                              & Debiasing / Feature Removal                                                                         & Downstream Classifier Accuracy                                                                           & Linear Classifier                                              & Yes                                                                     & No                                                                                      & Language Modelling    \\
\begin{tabular}[c]{@{}l@{}}CausaLM: Causal Model Explanation \\ Through Counterfactual Language Models\end{tabular} & \begin{tabular}[c]{@{}l@{}}Re-Training Model Copy \\ For Counterfactual Representation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Text representation-based individual\\ treatment effect (TReITE)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Retrained Base\\ Model\end{tabular} & Yes                                                                     & Yes                                                                                     & Sentiment Analysis    \\
Causal Concept Effect                                                                                               & Generative Modeling                                                                                 & Average Causal Effect Measure                                                                            & VAE                                                            & Yes                                                                     & Yes                                                                                     & Vision Classification \\
Concept Activation Vectors (TCAV)                                                                                   & Value Shift in Vector Direction                                                                     & Custom Gradient Sensitivity Measure                                                                      & Linear Classifier                                              & Yes                                                                     & Yes                                                                                     & Vision Classification \\
\begin{tabular}[c]{@{}l@{}}Latent Space Explanation \\ by Intervention\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}VAE Input Discretization \\ and Reconstruction\end{tabular}              & Reconstruction Quality                                                                                   & VAE                                                            & No                                                                      & \begin{tabular}[c]{@{}l@{}}Qualitative Judgement \\ (Vision Only)\end{tabular}          & Vision Classification \\
\begin{tabular}[c]{@{}l@{}}Meaningfully Explaining Model Mistakes \\ Using Conceptual Counterfactuals\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Weighted Combination of\\ Concept Vectors\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}Difference Between Concept\\ Addition and Removal Effect\end{tabular}         & Linear Classifier                                              & Yes                                                                     & Yes                                                                                     & Vision Classification \\ \bottomrule
\end{tabular}%
}
\end{table}
